Grounded Video Situation Recognition

Dense video understanding requires answering several questions such as who is doing what to whom, with what, how, why, and where. Recently, Video Situation Recognition (VidSitu) is framed as a task for structured prediction of multiple events, their relationships, and actions and various verb-role pairs attached to descriptive entities. This task poses several challenges in identifying, disambiguating, and co-referencing entities across multiple verb-role pairs, but also faces some challenges of evaluation. In this work, we propose the addition of spatio-temporal grounding as an essential component of the structured prediction task in a weakly supervised setting, and present a novel three stage Transformer model, VideoWhisperer, that is empowered to make joint predictions. In stage one, we learn contextualised embeddings for video features in parallel with key objects that appear in the video clips to enable fine-grained spatio-temporal reasoning. The second stage sees verb-role queries attend and pool information from object embeddings, localising answers to questions posed about the action. The final stage generates these answers as captions to describe each verb-role pair present in the video. Our model operates on a group of events (clips) simultaneously and predicts verbs, verb-role pairs, their nouns, and their grounding on-the-fly. When evaluated on a grounding-augmented version of the VidSitu dataset, we observe a large improvement in entity captioning accuracy, as well as the ability to localize verb-roles without grounding annotations at training time.

==> sections/6_checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes{} {\bf Briefly in the main paper, details in the appendix.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} {\bf Please see the project page}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes {\bf In Section 4, we described all the training details, we will also provide the model code.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes {\bf Most experiments in the ablation studies and SoTA comparison are repeated 3 to 10 times, standard deviation is reported.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? 
    \answerYes{} {\bf Section 4, implementation details.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes {\bf We use the VidSitu~\cite{sadhu2021vidsitu} dataset and augment it with grounding annotations for the proposed GVSR task.}
  \item Did you mention the license of the assets?
    \answerYes {\bf VidSitu~\cite{sadhu2021vidsitu} is publicly available and licensed under MIT license.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} {\bf We will add the grounding annotations over the existing VidSitu dataset on the project page.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{} {\bf The VidSitu dataset is publicly available for research purposes. Additional data collection did not require consent.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{} {\bf The VidSitu data does not contain PII information. It may have content that could be deemed to be offensive due to the nature of movies. Our new annotations do not add to this and are only used for evaluation.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes {\bf We add it in the Appendix.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{} {\bf Annotations were done in-house in the lab. No additional data was collected.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{} {\bf We add it in the Appendix.}
\end{enumerate}

\end{enumerate}


==> sections/guidelines.tex <==

\section{Submission of papers to NeurIPS 2021}

Please read the instructions below carefully and follow them faithfully.

\subsection{Style}

Papers to be submitted to NeurIPS 2021 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.

The margins in 2021 are the same as those in 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.

Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.

\subsection{Retrieval of style files}

The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2021.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.

The only supported style file for NeurIPS 2021 is \verb+neurips_2021.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}

The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.

\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.

The file \verb+neurips_2021.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.

The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2021+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2021}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2021/PaperInformation/FundingDisclosure}.

Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

\section*{References}

References follow the acknowledgments. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip

{
\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}


\section{Appendix}

Optionally include extra information (complete proofs, additional experiments and plots) in the appendix.
This section will often be part of the supplemental material.



==> tables/full-tables.tex <==
\begin{table}[t]
\begin{center}
\tabcolsep=0.12cm
\caption{Ablations on architecture. All the models use event-aware cross-attention. + indicates stages of the model. RV represents Role-Video decoder, RO is the Role-Object decoder, V is the Video encoder, VO is Video-Object encoder, and C is the Captioning Transformer.}
\label{tab:table1}
\begin{tabular}{llcccccc}
\toprule
\# & Architecture & Query & CIDEr & Rogue-L & Lea & IoU@0.3 & IoU@0.5 \\
\midrule
1 & RV + C & Role + GT-verb Emb & 48.03 & 41.98 & 55.60 & - & - \\ 
2 & RO + C & Role + GT-verb Emb & {\bf 69.08} & {\bf 45.59} & {\bf 48.30} & 0.21 & 0.08 \\
\midrule
3 & V + RO + C & Role + Event Emb & 68.08 & 45.20 & 46.11 & 0.23 & 0.11 \\
4 & VO + RO + C & Role + Event Emb & 68.23 & {\bf 45.58} & {\bf 48.22} & {\bf 0.27} & {\bf 0.15} \\
\bottomrule
\end{tabular}
\end{center}
\end{table} 




\begin{table}[h!]
\begin{center}
\caption{Ablation comparing different role query designs.}
\label{tab:table2}
\begin{tabular}{llcccccc}
\toprule
\# & Architecture & Query & CIDEr & Rogue-L & Lea & IoU@0.3 & IoU@0.5 \\
\midrule
1 & VO + RO + C & Role emb only & 66.42 & 45.67 & 46.63 & 0.27 & 0.11 \\ 
2 & VO + RO + C & Role + GT-verb Emb & 68.64 & 46.05 & 50.48 & 0.25 & 0.11 \\ 
3 & VO + RO + C & Role + Event Emb & 68.23 & 45.58 & 48.22 & 0.27 & 0.15 \\ 
\bottomrule
\end{tabular}
\end{center}
\end{table} 


\begin{table}[h!]
\begin{center}
\caption{Ablation on Cross-Attention in Role-Object decoder, in (VO+RO+C) with Role+Event embeddings as Role query.}
\label{tab:table3}
\begin{tabular}{l|c|c|c|c|c|}
\toprule
Architecture & Cider & Rogue-L & Lea & IoU@0.3 & IoU@0.5 \\
\midrule
Without Mask & 66.93 & 45.12 & 49.35 & 0.23 & 0.09 \\ 
With Mask  &68.23 &  45.58 & 48.22 & 0.27 & 0.15 \\ 
\bottomrule
\end{tabular}
\end{center}
\end{table} 





\begin{table}[h!]
\begin{center}
\caption{Verb Prediction}
\label{tab:table6}
\begin{tabular}{l|c|c|c|}
\toprule
Architecture & Acc@1 & Acc@5 & Rec@5 \\
\midrule
\multicolumn{4}{c|}{Verb Classification only} \\
\midrule
SlowFast baseline (separate events) \cite{sadhu2021vidsitu} & 46.79 & 75.90 & 23.38 \\
SlowFast (V) (Combined events) & 48.82 & 78.01 & 23.32 \\
SlowFast (VO) (Combined events)& 49.73 & 78.72 & 24.72 \\
\midrule
\multicolumn{4}{c|}{Verb + SRL training} \\
\midrule
SlowFast (V + RV + C) & 40.83 & 70.73 & 24.37 \\
SlowFast (VO + RV + C)  & 45.06 &  75.59 & 25.25 \\ 
\bottomrule
\end{tabular}
\end{center}
\end{table} 




\begin{table}[h!]
  \begin{center}
    \caption{Ablation on Role prediction in various settings. Role F1 is the F1 scores averaged over all the role classes. GT refers to using ground truth and Pred refers to using predicted verbs/roles for the task of SRL.}
    \label{tab:table5}
    \begin{tabular}{l|c|c|c|c|c|c|}
        \toprule
        Architecture & Verb & Role & Verb Acc@1 & Verb Recall@5 & Role F1 & CIDEr \\
        \midrule
        VidSitu \cite{sadhu2021vidsitu} & GT & GT & - & - & - & 46.01 \\
        VidSitu \cite{sadhu2021vidsitu} & GT & Pred & - & - & 0.88 & 45.52 \\
        VidSitu \cite{sadhu2021vidsitu} & Pred & GT mapped & 46.79 & 23.38 & - & 29.93 \\
        VidSitu \cite{sadhu2021vidsitu} & Pred & Pred & 46.79 & 23.38 & 0.47 & 30.33 \\
        \midrule
        RO+C & GT & GT &- & - & - & 0.6908 \\
        VO+RO+C & Pred &GT & 45.06 & 25.25 & - & 68.23 \\
        VO+RO+C & Pred & GT mapped & 45.06 & 25.25 & - & 51.24 \\
        VO+RO+C & Pred & Pred & 44.05 & 25.55 & 0.44 & 52.30 \\       
        \bottomrule
    \end{tabular}
  \end{center}
\end{table} 



\begin{table}[h!]
\tabcolsep=0.1cm
\caption{Results of GSRL on GVSR for end-to-end situation recognition.}
\label{tab:table7}
% \resizebox{\textwidth}{!}{
\begin{tabular}{lc ccccc cc}
\toprule
Architecture & Prediction & CIDEr & C-Vb & C-Arg & R-L & Lea & IoU@0.3 & IoU@0.5\\
\midrule
VidSitu \cite{sadhu2021vidsitu} & Verb + Role + SRL & 30.33 & 39.56 & 23.97 & 29.98 & 35.92 & - &- \\
\midrule
VO + RO + C & Verb + GT Role + SRL & 68.23 & 74.15 & 61.79 & 45.58 & 48.22 & 0.27 & 0.15 \\
VO + RO + C  & Verb + Role + SRL & 52.30 & 61.17 & 38.18 & 35.84 & 38.00 & 0.13 & 0.05 \\
\bottomrule
\end{tabular}
\end{table} 




%%%%%% SAME AS RESULT IN VERB PREDICTION TABLE %%%%%%
\begin{table}[h!]
  \begin{center}
    \caption{Results of Verb prediction on GVSR for end-to-end situation recognition.}
    \label{tab:table8}
    \begin{tabular}{l|c|c|c|c|}
        \toprule
        Architecture & Prediction & Acc@1 & Acc@5 & Rec@5 \\
        \midrule
        VidSitu \cite{sadhu2021vidsitu} & Verb + Role + SRL & 46.79  & 75.90 & 23.38 \\   
        \midrule
        VO + RO + C & Verb + GT Role + SRL & 45.06 & 75.59 & 25.25 \\
        VO + RO + C  & Verb + Role + SRL & 44.05 &  74.47 & 25.55 \\
        \bottomrule
    \end{tabular}
  \end{center}
\end{table} 



